Thermodynamic equilibrium of massless fermions with vorticity, chirality and magnetic field

The present thesis aimed to examine the effects of vorticity on the thermodynamics of relativistic quantum systems. We extend the Zubarev's non-equilibrium statistical operator method to address quantum effects induced by vorticity in the presence of chiral matter and external electromagnetic field and keeping full covariant and quantum properties of the system. To investigate the effects of vorticity, this work has been focused on systems consisting of massless chiral fermions. We recovered the significant quantum phenomena known in the literature, namely the chiral magnetic effect, the chiral vortical effect, the axial vortical effect and the chiral separation effect and we also revealed the presence of additional effects at second-order on thermal vorticity. This study has also identified and presented the exact solutions of thermal states for a system at global thermal equilibrium consisting of chiral massless fermions under the action of an external constant homogeneous magnetic field. Taking advantage of these exact solutions and conservation equations, the study also proved that the thermal coefficients related to first-order effects on thermal vorticity do not receive corrections from the external electromagnetic field. The same argument revealed existing relations between those thermal coefficients, even connecting coefficients related to vorticity to other related to electromagnetic field. For instance, this analysis has found that the chiral vortical effect and the chiral magnetic effect conductivities are connected one to the other by a differential equation. Therefore, this research provides the first steps into deriving the relations between the effects and the interplay of electromagnetic fields and vorticity.

==> AppCVEMagnetic.tex <==
%*********************************************************************************
\chapter{Chiral vortical effect in magnetic field}
%*********************************************************************************
\label{ch:CVEInB}
Here we report the calculations of chiral vortical effect with Ritus method.
The CVE conductivity at first order on thermal vorticity is given by:
%
\begin{equation}
\label{eq:CVEinBPieces}
\begin{split}
C\apic{J}_{02|3|1}=&\int_X\, \mean{\h{T}_{02}(x)\h{j}_3(0)}\frac{x_1}{\beta},\\
C\apic{J}_{01|3|2}=&\int_X\, \mean{\h{T}_{01}(x)\h{j}_3(0)}\frac{x_2}{\beta},\\
C\apic{B}_{0|3}=&\frac{B}{2}\int_X\, \mean{\h{j}_0(x)\h{j}_{3}(0)}\frac{(x_2)^2}{\beta},\\
W\apic{V}=&\mycorr{\,\h J_3\, \h j_3\,}\ped{LRF}=C\apic{J}_{02|3|1}-C\apic{J}_{01|3|2}-C\apic{B}_{0|3}.
\end{split}
\end{equation}
%
where $\h{T}$ is the stress-energy tensor of free Dirac field.
First we write the operators in Euclidean space-time and using the point-splitting procedure (as in Sec~\ref{subsec:pointsplit}):
%
\begin{equation*}
\begin{split}
\h T_{\mu\nu}(X)&=\lim_{X_1,X_2\to X} \mathcal{D}_{\mu\nu}(\de_{X_1},\de_{X_2})_{ab}\,\h{\bar{\psi}}_a(X_1)\h{\psi}_b(X_2),\\
\h{j}_\rho(Y)&=\lim_{Y_1,Y_2\to Y} (-\ii)^{1-\delta_{\rho,0}}\left(\gamma_\rho\right)_{cd}\,\h{\bar{\psi}}_c(Y_1)\h{\psi}_d(Y_2).
\end{split}
\end{equation*}
%
where all the gamma matrices are Euclidean matrices and
%
\begin{equation*}%\label{fermD}
\mathcal{D}_{\mu\nu} (\partial_{X_1},\partial_{X_2})=
\frac{\I^{\delta_{0\mu}+\delta_{0\nu}}}{4}\left[ \gamma_\mu (\partial_{X_2}-\partial_{X_1})_\nu
	+\gamma_\nu (\partial_{X_2}-\partial_{X_1})_\mu\right].
\end{equation*}
%
In this form, using Wick theorem we have
%
\begin{equation*}
\begin{split}
\mean{\,\h T_{\mu\nu}(X)\,\h j_\rho(0)}\ped{B,c}=&\lim_{\substack{X_1 X_2\to X\\Y_1 Y_2\to 0}}(-\ii)^{1-\delta_{\rho,0}}\left(\gamma_\rho\right)_{cd}
	\mathcal{D}_{\mu\nu}(\de_{X_1},\de_{X_2})_{ab}\times\\
&\times\mean{\h{\bar{\psi}}_a(X_1)\h{\psi}_d(Y_2)}\ped{B} \mean{\h{\psi}_b(X_2)\h{\bar{\psi}}_c(Y_1)}\ped{B}.
\end{split}
\end{equation*}
%
The propagator of Fermion field is not expressed as linear plane wave but with Ritus operators $E_p(X)$ defined in Eq.~(\ref{eq:defE})
%
\begin{equation*}
\mean{\bar{\Psi}(X)_a \Psi(Y)_b}\ped{B}=-\sumint_{\h P}\sum_\chi E_{\h p}(Y)_{bb'}
	\left(\mathbb{P}_\chi\frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2} \right)_{b'a'} \bar{E}_{\h p}(X)_{a'a};
\end{equation*}
%
therefore we have to determine how the linear first order derivatives in $\mathcal{D}_{\mu\nu}$ acts on the propagators:
%
\begin{equation*}
{\de_Y}_\mu \mean{\bar{\Psi}(X)_a \Psi(Y)_b}\ped{B}=-\sumint_{\h P}\sum_\chi {\de_Y}_\mu E_{\h p}(Y)_{bb'}
	\left(\mathbb{P}_\chi\frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2} \right)_{b'a'} \bar{E}_{\h p}(X)_{a'a}.
\end{equation*}
%
We recall that $E_{\h p}(X)=\sum'_{\sigma=\pm}E_{\h{p}\sigma}(X)\Delta(\sigma)$ from which follows
%
\begin{equation*}
\begin{split}
{\de_X}_\mu E_{\h{p}\sigma}(X)&={\de_X}_\mu\left[N(n)\e^{\I(P_0\tau+P_2 X_2+P_3 X_3)}D_n\left((X_1-P_2/qB)\sqrt{2|qB|}\right) \right]\\
&=\begin{cases} \I P_\mu E_{\h{p}\sigma}(X) & \mu\neq 1\\
				N(n)\e^{\I(P_0\tau+P_2 X_2+P_3 X_3)}\frac{\de}{\de X_1}D_n\left((X_1-P_2/qB)\sqrt{2|qB|}\right) &\mu=1
\end{cases}
\end{split}
\end{equation*}
%
Using the parabolic cylinder functions property
%
\begin{equation*}
\frac{\de}{\de \rho}D_n(\rho)=\frac{n}{2} D_{n-1}(\rho)-\frac{1}{2}D_{n+1}(\rho)
\end{equation*}
%
and calling $\rho=(X_1-P_2/qB)\sqrt{2|qB|}$ we have
%
\begin{equation*}
\frac{\de}{\de X_1}D_n\left((X_1-P_2/qB)\sqrt{2|qB|}\right)=\frac{\de\rho}{\de X_1}\frac{\de}{\de\rho}D_n(\rho)=
\sqrt{2|qB|}\frac{n}{2}D_{n-1}(\rho)-\sqrt{2|qB|}\frac{1}{2}D_{n+1}(\rho).
\end{equation*}
%
We have the basic set-up to compute the CVE conductivity. In the next section we compute every piece in Eq.~(\ref{eq:CVEinBPieces}).

%*********************************************************************************
\section{\texorpdfstring{$C\apic{J}_{02|3|1}$}{CJ02|3|1}}
%*********************************************************************************
The derivative of Fermionic propagator in the correlators $C_{02|3|1}\apic{J}$ follows a simple rule,
indeed since both the index of stress-energy tensor $\mu$ and $\nu$ are different from one, we have
%
\begin{equation*}
\begin{split}
\mean{\,\h T_{\mu\nu}(X)&\,\h j_\rho(0)}\ped{B,c}=-\lim_{\substack{X_1 X_2\to X\\Y_1 Y_2\to 0}}(-\ii)^{1-\delta_{\rho,0}}\sumint_{\h P,\h Q}\sum_{\chi,\chi'}
	\left(\gamma_\rho\right)_{cd}\mathcal{D}_{\mu\nu}(-\I P,\I Q)_{ab}\times\\
	&\times E_{\h p}(Y_2)_{dd'} \left(\mathbb{P}_\chi\frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2} \right)_{d'a'} \bar{E}_{\h p}(X_1)_{a'a}
	 E_{\h q}(X_2)_{bb'} \left(\mathbb{P}_{\chi'}\frac{-\I\slashed{\underline{Q}}_{\chi'}^+}{{\underline{Q}^+_{\chi'}}^2} \right)_{b'c'} \bar{E}_{\h q}(Y_1)_{c'c}\\
=& -(-\ii)^{1-\delta_{\rho,0}}\sumint_{\h P,\h Q}\sum_{\chi,\chi'} \tr\left[\mathcal{D}_{\mu\nu}(-\I P,\I Q)E_{\h q}(X)
	\mathbb{P}_{\chi'}\frac{-\I\slashed{\underline{Q}}_{\chi'}^+}{{\underline{Q}^+_{\chi'}}^2}\bar{E}_{\h q}(0)\gamma_\rho
	E_{\h p}(0)\mathbb{P}_\chi\frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\bar{E}_{\h p}(X) \right].
\end{split}
\end{equation*}
%
We can use the $\gamma_5$ anti-commutation properties to move the projector $\mathbb{P}_\chi$:
%
\begin{equation*}
\begin{split}
\mean{\,\h T_{\mu\nu}(X)\,\h j_\rho(0)}\ped{B,c}
=& -(-\ii)^{1-\delta_{\rho,0}}\sumint_{\h P,\h Q}\sum_{\chi} \tr\left[\mathcal{D}_{\mu\nu}(-\I P,\I Q)E_{\h q}(X)
	\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}\bar{E}_{\h q}(0)\gamma_\rho\times\right.\\
	&\left.\times E_{\h p}(0)\frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\bar{E}_{\h p}(X) \right]\\
=& -(-\ii)^{1-\delta_{\rho,0}}\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_3,\sigma_4=\pm}
	E_{\h q\sigma_4}(X)E^*_{\h p\sigma_1}(X)E^*_{\h q\sigma_3}(0)E_{\h p\sigma_2}(0)\times\\
	&\times\tr\left[\mathcal{D}_{\mu\nu}(-\I P,\I Q)\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_3) \gamma_\rho \Delta(\sigma_2) \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\Delta(\sigma_1) \right].
\end{split}
\end{equation*}
%
where $\sigma_1=\sigma_2=\bar\sigma=$sgn$(qB)$ when $l_p=0$ and $\sigma_3=\sigma_4=\bar\sigma$ when $l_q=0$.
We now set the indices $\mu=0,\,\nu=2,\,\rho=3,\,i=1$, then we can take advantage of $[\gamma_3,\Delta(\sigma_2)]=0$
and of $\Delta(\sigma_3)\Delta(\sigma_2)=\delta_{\sigma_3,\sigma_2}\Delta(\sigma_2)$ to remove the sum on $\sigma_3$
%
\begin{equation*}
\begin{split}
\mean{\,\h T_{02}(X)\,\h j_3(0)}\ped{B,c}
=& \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_4=\pm}
	E_{\h q\sigma_4}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)\\
&\tr\left[\Delta(\sigma_1)\mathcal{D}_{02}(-\I P,\I Q)\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_2) \gamma_3 \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2} \right],
\end{split}
\end{equation*}
%
where $\sigma_1=\sigma_2=\bar\sigma$ when $l_p=0$ and $\sigma_2=\sigma_4=\bar\sigma$ when $l_q=0$.
We then split $\mathcal{D}_{02}$ in two terms, one linear in $\gamma_0$ and the other linear in $\gamma_2$:
%
\begin{equation*}
\mathcal{D}_{02}(-\I P,\I Q)=-\frac{p_2+q_2}{4}\gamma_0-\frac{p_0+q_0}{4}\gamma_2,
\end{equation*}
%
consequently we split the correlator into the corresponding parts:
%
\begin{equation*}
C\apic{J}_{02|3|1}=\tilde{C}_{0|3|1}+\tilde{C}_{2|3|1}.
\end{equation*}
%
Then because $\Delta(\sigma_1)$ and $\gamma_0$ commutes we obtain
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}=&- \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X \frac{x_1}{\beta}
	\frac{E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{Q}^+_{\chi}}^2{\underline{P}^+_\chi}^2}\times\\
&\times\frac{p_2+q_2}{4}\tr\left[\gamma_0\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
	\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right],
\end{split}
\end{equation*}
%
where $\sigma_1=\sigma_2=\bar\sigma$ when $l_p=0$ and $\sigma_2=\sigma_1=\bar\sigma$ when $l_q=0$.
Similarly from $\Delta(\sigma_1)\gamma_2=-\gamma_2\Delta(\sigma_1)$ we have
%
\begin{equation*}
\begin{split}
\tilde{C}_{2|3|1}=& -\ii\sideset{}{'}\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X \frac{x_1}{\beta}
	\frac{E_{\h q-\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{Q}^+_{\chi}}^2{\underline{P}^+_\chi}^2}\times\\
&\times\frac{p_0+q_0}{4}\tr\left[\gamma_2\Delta(-\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
	\Delta(\sigma_2) \gamma_3\left(-\I\slashed{\underline{P}}_\chi^+\right) \right],
\end{split}
\end{equation*}
%
where now $\sigma_1=\sigma_2=\bar\sigma$ when $l_p=0$ and $\sigma_2=-\sigma_1=\bar\sigma$ when $l_q=0$. For this part we putted a prime
also on the sum on momenta because when both $l_p$ and $l_q$ are $0$ the result is vanishing because of the Kronecker delta
$\delta_{\sigma_1,-\sigma_4}$ we simplified. Notice that the coordinate dependence is only contained in the eigenfunctions $E$.
Both for $\tilde{C}_{0|3|1}$ and $\tilde{C}_{2|3|1}$ if we integrate in $\tau$ and $x_3$ we would obtain $\delta_{p_0,q_0}\delta(p_3-q_3)$;
therefore when evaluating the trace we set $q_0=p_0$ and $q_3=p_3$. After we removed the odd part in $p_3$, which is vanishing after
integrating in $p_3$, we obtain the traces:
%
\begin{equation*}
\begin{split}
F_{03}\equiv&\tr\left[\gamma_0\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
		\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right]\\
	=&-\frac{\I}{2}\chi\left[\sigma_1\left(p_0^2-p_3^2+\underline{P}_2\underline{Q}_2\right)+\sigma_2\left(p_0^2-p_3^2-\underline{P}_2\underline{Q}_2 \right) \right], \\
F_{23}\equiv&\tr\left[\gamma_2\Delta(-\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
		\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right]
	=-\frac{\I p_0}{2}\chi\left[\sigma_1\left( \underline{Q}_2-\underline{P}_2\right)+\sigma_2\left( \underline{P}_2+\underline{Q}_2\right) \right],
\end{split}
\end{equation*}
%
where we remind that the underline symbol under momenta stands for
%
\begin{equation*}
\underline{P}=\{p_0,0,\underline{P}_2=-\bar\sigma\sqrt{2|qB|l_p},p_3\},\quad \underline{Q}=\{p_0,0,\underline{Q}_2=-\bar\sigma\sqrt{2|qB|l_q},p_3\}.
\end{equation*}
%
The non-trivial integrals are those in $x_1$ and in $p_2$ because the functions $E_{\hat{p}\sigma}(X)$, defined in Eq.~(\ref{eq:defEpsigma}),
depend on them through the argument of parabolic cylinder functions $D_n(\rho)$. Before dealing with those integrals in order to simplify
the notation we first define some auxiliary functions $\mathcal{I}^0_{03}$ and $\mathcal{I}^0_{02}$:
%
\begin{equation*}
\begin{split}
(2\pi)^3\delta_{p_0,q_0}\delta(p_2-q_2)\delta(p_3-q_3)\mathcal{I}_{03}\equiv&
	\int \frac{\D p_2}{2\pi}\int_X E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0) \frac{x_1}{\beta}p_2\\
(2\pi)^3\delta_{p_0,q_0}\delta(p_2-q_2)\delta(p_3-q_3)\mathcal{I}_{23}\equiv&
	\int \frac{\D p_2}{2\pi}\int_X E_{\h q-\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0) \frac{x_1}{\beta}.
\end{split}
\end{equation*}
%
Replacing the form~(\ref{eq:defEpsigma}) of the functions $E_{\hat{p}\sigma}(X)$, the previous functions read:
%
\begin{equation*}
\begin{split}
 \mathcal{I}_{03}=&
	\frac{2|qB|}{\sqrt{n_p!n_q!\tilde{n}_p!\tilde{n}_q!}}
		\int \D p_2 \int \D x_1 p_2 x_1 D_{n_p}(\rho)D_{\tilde{n}_p}(-y) D_{n_q}(\rho) D_{\tilde{n}_q}(-y_q),\\
\mathcal{I}_{23}=&
	\frac{2|qB|}{\sqrt{n_p!n_q^-!\tilde{n}_p!\tilde{n}_q!}}
		\int \D p_2 \int \D x_1\,x_1 D_{n_p}(\rho)D_{\tilde{n}_p}(-y) D_{n_q^-}(\rho) D_{\tilde{n}_q}(-y_q),
\end{split}
\end{equation*}
%
where we denoted
%
\begin{equation*}
\begin{split}
n_p=&l_p+\sigma_1\bar\sigma/2-1/2,\quad n_q=l_q+\sigma_1\bar\sigma/2-1/2,\quad n_q^-=l_q-\sigma_1\bar\sigma/2-1/2,\\
\tilde{n}_p=&l_p+\sigma_2\bar\sigma/2-1/2,\quad \tilde{n}_q=l_q+\sigma_2\bar\sigma/2-1/2,\\
\rho=&\sqrt{2|qB|}\left(x_1-\frac{p_2}{qB}\right),\quad y=\frac{\sqrt{2|qB|}}{qB}p_2.
\end{split}
\end{equation*}
%
Using the recurrence relations
%
\begin{align*}
z D_\nu(z)&=D_{\nu+1}(z)+\nu D_{\nu-1}(z)\\
z^2 D_\nu(z)&=D_{\nu+2}(z)+(2\nu+1)D_\nu(z)+\nu(\nu-1) D_{\nu-2}(z)
\end{align*}
%
we obtain
%
\begin{equation*}
\begin{split}
\mathcal{I}_{03}=& \frac{qB}{2} \left[ -\delta_{l_p,l_q-1}\sqrt{n_p+1}\sqrt{\tilde{n}_p+1} +\delta_{l_p,l_q}(2\tilde{n}_p+1) 
	-\delta_{l_p,l_q+1}\sqrt{n_p}\sqrt{\tilde{n}_p}   \right],\\
\mathcal{I}_{23}=& \frac{|qB|}{\sqrt{2|qB|}}\Big[\delta_{l_p,l_q}\left(\delta_{\sigma_1,-\bar\sigma}\sqrt{n_p+1}+\delta_{\sigma_1,\bar\sigma}\sqrt{n_p}\right)
	-\delta_{l_p+1,l_q}\delta_{\sigma_1,\bar\sigma}\sqrt{\tilde{n}_p+1}-\delta_{l_p-1,l_q}\delta_{\sigma_1,-\bar\sigma}\sqrt{\tilde{n}_p}\Big].
\end{split}
\end{equation*}
%
In terms of these functions the parts of the correlator we are computing become
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}=& -\frac{\ii T}{2}\sum_{\chi}\int\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\sum_{l_p,l_q=0}^\infty\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}
	\frac{\mathcal{I}_{03}\,F_{03}}{\Gamma(l_p)\Gamma(l_q)},\\
\tilde{C}_{2|3|1}= & -\frac{\ii T}{2}\sum_{\chi}\int\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\sideset{}{'}\sum_{l_p,l_q=0}^\infty\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}
	\frac{\mathcal{I}_{23}\, p_0\, F_{23}}{\Gamma(l_p)\Gamma(l_q)},
\end{split}
\end{equation*}
%
where we also defined
%
\begin{equation*}
\Gamma(l)\equiv p_0^2+p_3^2+2|qB|l
\end{equation*}
%
and where the primes on the sums reminds the constraints:
%
\begin{equation*}
\text{for }\tilde{C}_{0|3|1}\,\begin{cases}l_p=0\rightarrow\, \sigma_1=\bar{\sigma},\,\sigma_2=\bar{\sigma}\\
	 l_q=0\rightarrow\, \sigma_1=\bar{\sigma},\,\sigma_2=\bar{\sigma}\end{cases},\quad
\text{for }\tilde{C}_{2|3|1}\,\begin{cases}l_p=0\rightarrow\, \sigma_1=-\bar{\sigma},\,\sigma_2=\bar{\sigma},\,l_q>0\\
	l_q=0\rightarrow\, \sigma_1=\bar{\sigma},\,\hphantom{-}\sigma_2=\bar{\sigma},\,l_p>0\end{cases}.
\end{equation*}
%

Consider the sums on $l_p$ and $l_q$ in $\tilde{C}_{0|3|1}$; when $l_p=0$ we have $\sigma_1=\sigma_2=\bar\sigma$ and for $\mathcal{I}_{03}$ only
the terms with $l_q=0,1$ are non vanishing:
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}^{l_p=0}=& \frac{|qB| T}{4}\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)} \left[\frac{1}{\Gamma(1)}-\frac{1}{\Gamma(0)} \right]\\
=& \frac{|qB| T}{2}\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)} \left[\frac{1}{\Gamma(1)}-\frac{1}{\Gamma(0)} \right]\\
=& \frac{|qB|T}{2}\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)},
\end{split}
\end{equation*}
%
where we used the fact that after the Matsubara sum, integration on $p_3$ and sum on $\chi$ the last term is vanishing.
When $l_p>0$ and $l_q=0$ we have $\sigma_1=\sigma_2=\bar\sigma$ and only the term with $l_p=1$ can contribute:
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}^{l_p>0,l_q=0}=& \frac{|qB| T}{4}\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)}\\
=& \frac{|qB| T}{2}\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)}
\end{split}
\end{equation*}
%
that is, it is equivalent to the case $l_p=0$; the sum of the two gives
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}^{l_p=0}+\tilde{C}_{0|3|1}^{l_p>0,l_q=0}&=|qB| T\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)}.
\end{split}
\end{equation*}
%
When $l_p,l_q>0$ the sums on $\sigma_1,\sigma_2$ give
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}^{l_p>0,l_q>0}=& \frac{T|qB|}{4}\sum_{l_p=1}^\infty \sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\frac{1}{\Gamma(l_p)}
	 \Bigg[\frac{p_0^2-p_3^2}{\Gamma(l_p+1)}-\frac{2(p_0^2-p_3^2-2|qB|l_p)}{\Gamma(l_p)}\\
	 &+\frac{(1-\delta_{l_p,1})(p_0^2-p_3^2)}{\Gamma(l_p-1)}\Bigg]\\
=& T|qB|\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\Bigg[\frac{p_0^2-p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}-\frac{p_0^2-p_3^2-2|qB|l_p}{\Gamma(l_p)^2}\Bigg].
\end{split}
\end{equation*}
%
The coefficient $\tilde{C}_{0|3|1}$ is then
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|1}=&|qB| T\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\Bigg\{
	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)}+\sum_{l_p=1}^\infty\Bigg[\frac{p_0^2-p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}-\frac{p_0^2-p_3^2-2|qB|l_p}{\Gamma(l_p)^2}\Bigg]\Bigg\}.
\end{split}
\end{equation*}
%

We turn now to $\tilde{C}_{2|3|1}$. For $l_q=0$ it easy to check that $\mc{I}_{23}$ is always vanishing. The same holds for $l_p=0$.
We then have only the case $l_p>0$ and $l_q>0$; the sums in $\sigma_1$ and $\sigma_2$ give
%
\begin{equation*}
\begin{split}
\tilde{C}_{2|3|1}=&\,\tilde{C}_{2|3|1}^{l_p>0,l_q>0}=
		-\frac{T|qB|}{2}\sum_{l_p=1}^\infty \sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\frac{p_0^2}{\Gamma(l_p)} \Big[\frac{1}{\Gamma(l_p+1)}+\frac{1-\delta_{l_p,1}}{\Gamma(l_p-1)}\Big]\\
=& |qB|T\sum_{\chi}\chi\int_{0}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\Bigg\{\sum_{l_p=1}^\infty
	\frac{-2 p_0^2}{\Gamma(l_p)} \frac{1}{\Gamma(l_p+1)}\Bigg\}.
\end{split}
\end{equation*}
%
In total the correlator is
%
\begin{equation*}
\begin{split}
C\apic{J}_{02|3|1}=&|qB| T\sum_{\chi}\chi\!\int_{0}^\infty\!\!\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\!\Bigg\{\! \frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)}
	+\!\sum_{l_p=1}^\infty\!\Bigg[\frac{-p_0^2-p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}-\frac{p_0^2-p_3^2-2|qB|l_p}{\Gamma(l_p)^2}\Bigg]\Bigg\}.
\end{split}
\end{equation*}
%

%*********************************************************************************
\section{\texorpdfstring{$C\apic{J}_{01|3|2}$}{CJ01|3|2}}
%*********************************************************************************
To evaluate the correlator $C\apic{J}_{01|3|2}$ we first split $\mathcal{D}$ in two part, one linear in $\gamma_0$ and one
linear in $\gamma_1$. The part in $\gamma_1$ contains the derivative $\de_0$ which act on the exponential and can be done
as in the previous section. The part linear in $\gamma_0$ contains a derivative respect to $x$ direction that gives
$\de_1 E^*_{p\sigma_1}(X)$ and $\de_1 E_{q\sigma_4}(X)$. We then define three pieces
%
\begin{equation*}
C\apic{J}_{01|3|2}=\tilde{C}^{(1)}_{0|3|2}+\tilde{C}^{(2)}_{0|3|2}+\tilde{C}_{1|3|2},
\end{equation*}
%
with
%
\begin{equation*}
\begin{split}
\tilde{C}^{(1)}_{0|3|2}=&- \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_3,\sigma_4=\pm}\int_X\frac{x_2}{\beta}
	E_{\h q\sigma_4}(X)E^*_{\h q\sigma_3}(0)E_{\h p\sigma_2}(0)\de_1 E^*_{\h p\sigma_1}(X)\times\\
&\times\frac{\I}{4}\tr\left[\gamma_0\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_3) \gamma_3 \Delta(\sigma_2) \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\Delta(\sigma_1) \right];\\
\tilde{C}^{(2)}_{0|3|2}=& \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_3,\sigma_4=\pm}\int_X\frac{x_2}{\beta}
	\de_1 E_{\h q\sigma_4}(X)E^*_{\h q\sigma_3}(0)E_{\h p\sigma_2}(0)E^*_{\h p\sigma_1}(X)\times\\
&\times\frac{\I}{4}\tr\left[\gamma_0\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_3) \gamma_3 \Delta(\sigma_2) \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\Delta(\sigma_1) \right];\\
\tilde{C}_{1|3|2}=&\ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_3,\sigma_4=\pm}\int_X\frac{x_2}{\beta}
	E_{\h q\sigma_4}(X)E^*_{\h q\sigma_3}(0)E_{\h p\sigma_2}(0)E^*_{\h p\sigma_1}(X)\times\\
&\times\frac{-(q_0+p_0)}{4}\tr\left[\gamma_1(q_0+p_0)\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_3) \gamma_3 \Delta(\sigma_2) \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\Delta(\sigma_1) \right].
\end{split}
\end{equation*}
%
Now, as before we take advantage of the fact that $\Delta(\sigma)$ commutes with $\gamma_0$ and $\gamma_3$ but that it anti-commutes with $\gamma_1$:
%
\begin{equation*}
\begin{split}
\tilde{C}^{(1)}_{0|3|2}=&- \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X\frac{x_2}{\beta}
	\frac{E_{\h q\sigma_1}(X)\de_1 E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{P}^+_\chi}^2 {\underline{Q}^+_{\chi}}^2}\times\\
&\times\frac{\I}{4}\tr\left[\gamma_0\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
	\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right];\\
\tilde{C}^{(2)}_{0|3|2}=& \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X\frac{x_2}{\beta}
	\frac{\de_1 E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X)E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{P}^+_\chi}^2 {\underline{Q}^+_{\chi}}^2}\times\\
&\times\frac{\I}{4}\tr\left[\gamma_0\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
	\times\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right];\\
\tilde{C}_{1|3|2}=& \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X\frac{x_2}{\beta}
	\frac{E_{\h q\sigma_1}(X)E^*_{\h p-\sigma_1}(X)E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{P}^+_\chi}^2 {\underline{Q}^+_{\chi}}^2}\times\\
&\times\frac{-(q_0+p_0)}{4}\tr\left[\gamma_1\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
	\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right].
\end{split}
\end{equation*}
%
The space integral for all the three pieces creates a term $-\I\delta_{p_0,q_0}\delta'(p_2-q_2)\delta(p_3-q_3)$, therefore when
evaluating the trace we can set $q_0=p_0,\,q_3=p_3$ and after removing odd parts in $p_3$ we obtain:
%
\begin{equation*}
\begin{split}
F_{03}=&-\frac{\I}{2}\chi\left[\sigma_1\left(p_0^2-p_3^2+\underline{P}_2\underline{Q}_2\right)+\sigma_2\left(p_0^2-p_3^2-\underline{P}_2\underline{Q}_2 \right) \right]\\
F_{13}=&\tr\left[\gamma_1\Delta(\sigma_1)\mathbb{P}_{\chi}\left(-\I\slashed{\underline{Q}}_{\chi}^+\right)
\Delta(\sigma_2) \gamma_3 \left(-\I\slashed{\underline{P}}_\chi^+\right) \right] = 
\frac{\chi}{2}p_0\left[\underline{P}_2(\sigma_1\sigma_2+1)+\underline{Q}_2(\sigma_1\sigma_2-1)\right].
\end{split}
\end{equation*}
%
Now we define the following integrals
%
\begin{equation*}
\begin{split}
(2\pi)^2\delta_{p_0,q_0}\delta(p_3-q_3)\mathcal{I}^1_{03}\equiv&
\int_X \int\frac{\D p_2}{2\pi}\int\frac{\D q_2}{2\pi} E_{\h q\sigma_1}(X)\de_1 E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)\frac{x_2}{\beta}\\
(2\pi)^2\delta_{p_0,q_0}\delta(p_3-q_3)\mathcal{I}^2_{03}\equiv&
\int_X \int\frac{\D p_2}{2\pi}\int\frac{\D q_2}{2\pi} \de_1 E_{\h q\sigma_1}(X) E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)\frac{x_2}{\beta},\\
(2\pi)^2\delta_{p_0,q_0}\delta(p_3-q_3)\mathcal{I}_{13}\equiv&
\int_X \int\frac{\D p_2}{2\pi}\int\frac{\D q_2}{2\pi} E_{\h q\sigma_1}(X) E^*_{\h p-\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)\frac{x_2}{\beta}.
\end{split}
\end{equation*}
%
The results of integration are
%
\begin{equation*}
\begin{split}
\mathcal{I}^1_{03}&(l_p,l_q,\sigma_1,\sigma_2)=
\frac{qB\I}{2}\left[\delta_{l_q,l_p}\left(2n_p+1\right)-\delta_{l_q,l_p-1}\sqrt{n_p\tilde{n}_p}-\delta_{l_q,l_p+1}\sqrt{(n_p+1)(\tilde{n}_p+1)}\right],\\
\mathcal{I}^2_{03}&(l_p,l_q,\sigma_1,\sigma_2)=-\mathcal{I}^1_{03}(l_p,l_q,\sigma_1,\sigma_2),\\
\mathcal{I}_{13}& =\!\I\sqrt{\frac{|qB|}{2}}\bar\sigma\!\l[\!\delta_{l_p,l_q}\!\l(\delta_{\sigma_1,\bar\sigma}\sqrt{n_p+1}-\delta_{\sigma_1,-\bar\sigma}\sqrt{n_p} \r)
	\!\!+\delta_{l_p,l_q-1}\delta_{\sigma_1,-\bar\sigma}\sqrt{\tilde{n}_p+1}-\!\delta_{l_p,l_q+1}\delta_{\sigma_1,\bar\sigma}\sqrt{\tilde{n}_p}\r].
\end{split}
\end{equation*}
%
Consequently we have to compute
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|2}\equiv&\,\tilde{C}^{(1)}_{0|3|2}+\tilde{C}^{(2)}_{0|3|2}=
\frac{T}{2}\sum_{\chi}\int\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\sum_{l_p,l_q=0}^\infty\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}
\frac{\mathcal{I}^1_{03}F_{03}}{{\Gamma(l_p)}{\Gamma(l_q)}},\\
\tilde{C}_{1|3|2}= & -\frac{\ii T}{2}\sum_{\chi}\int\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\sum_{l_p,l_q=0}^\infty\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}
\frac{\mathcal{I}_{13} p_0 F_{13}}{{\Gamma(l_p)}{\Gamma(l_q)}}.
\end{split}
\end{equation*}
%

Consider $\tilde{C}_{0|3|2}$, for $l_p=0$ we have
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|2}^{l_p=0}=&-\frac{|qB|T}{4}\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}\frac{p_0^2-p_3^2}{{\Gamma(0)}}
	\left[\frac{1}{{\Gamma(1)}}-\frac{1}{{\Gamma(0)}} \right]\\
=&-\frac{|qB|T}{2}\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)},
\end{split}
\end{equation*}
%
while for $l_p>0$ and $l_q=0$ we have
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|2}^{l_p>0,l_q=0}=&-\frac{|qB|T}{2}\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(0)\Gamma(1)},
\end{split}
\end{equation*}
%
and at last for $l_p,l_q>0$ we find
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|2}^{l_p>0,l_q>0}
=& -\frac{|qB|T}{4}\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}\frac{1}{{\Gamma(l_p)}}
		\bigg[-2\frac{p_0^2-p_3^2+2|qB|l_p}{{\Gamma(l_p)}}\\
	&+\frac{p_0^2-p_3^2}{{\Gamma(l_p+1)}} +(1-\delta_{l_p,1})\frac{p_0^2-p_3^2}{{\Gamma(l_p-1)}}\Bigg]\\
=& |qB|T\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\bigg[\frac{-p_0^2+p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}+\frac{p_0^2-p_3^2+2|qB|l_p}{\Gamma(l_p)^2}\bigg].
\end{split}
\end{equation*}
%
Summing all the pieces we obtain
%
\begin{equation*}
\begin{split}
\tilde{C}_{0|3|2}=& |qB|T\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}\Bigg\{\frac{-p_0^2+p_3^2}{\Gamma(0)\Gamma(1)}
	+\sum_{l_p=1}^\infty\bigg[\frac{-p_0^2+p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}+\frac{p_0^2-p_3^2+2|qB|l_p}{\Gamma(l_p)^2}\bigg]\Bigg\}.
\end{split}
\end{equation*}
%

Consider now $\tilde{C}_{1|3|2}$;  for $l_p=0$ we have $\tilde{C}_{1|3|2}^{l_p=0}=0$. For $l_p>0$ and $l_q=0$ instead it reads 
%
\begin{equation*}
\begin{split}
\tilde{C}_{1|3|2}^{l_p>0,l_q=0}=&T\frac{|qB|}{2}\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2}{{\Gamma(0)}{\Gamma(1)}}\\
=&T|qB|\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\frac{p_0^2}{{\Gamma(0)}{\Gamma(1)}}.
\end{split}
\end{equation*}
%
When $l_p>0$ and $l_q>0$ it is
%
\begin{equation*}
\begin{split}
\tilde{C}_{1|3|2}^{l_p>0,l_q>0}=& T\frac{|qB|}{2}\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}
	\frac{p_0^2}{{\Gamma(l_p)}}\Big\{\frac{1}{{\Gamma(l_p+1)}}+(1-\delta_{l_p,1})\frac{1}{{\Gamma(l_p-1)}}\Big\}\\
=& T|qB|\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2}	T\sum_{\{p_n\}}	\frac{2 p_0^2}{{\Gamma(l_p)}{\Gamma(l_p+1)}},
\end{split}
\end{equation*}
%
for a total of
%
\begin{equation*}
\begin{split}
\tilde{C}_{1|3|2}=&|qB|T\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\Bigg\{
	\frac{p_0^2}{{\Gamma(0)}{\Gamma(1)}}+ \sum_{l_p=1}^\infty\frac{2 p_0^2}{{\Gamma(l_p)}{\Gamma(l_p+1)}}\Bigg\}.
\end{split}
\end{equation*}
%
The whole correlators is
%
\begin{equation*}
\begin{split}
C\apic{J}_{01|3|2}=&|qB|T\sum_{\chi}\chi\!\int_0^\infty\!\!\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\!\Bigg\{\!	\frac{p_3^2}{{\Gamma(0)}{\Gamma(1)}}+
	 \!\sum_{l_p=1}^\infty\bigg[\frac{p_0^2+p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}+\frac{p_0^2-p_3^2+2|qB|l_p}{\Gamma(l_p)^2}\bigg]\Bigg\}.
\end{split}
\end{equation*}
%

%*********************************************************************************
\section{\texorpdfstring{$C\apic{B}_{0|3}$}{CB0|3}}
%*********************************************************************************
For the coefficient $C\apic{B}_{0|3}$ we have to compute the correlator $\mean{\,\h j_{\mu}(X)\,\h j_\rho(0)}\ped{B,c}$
which does not involves any derivatives, therefore we find:
%
\begin{equation*}
\begin{split}
\mean{\,\h j_{\mu}(X)\,\h j_\rho(0)}\ped{B,c}
=& -(-\ii)^{2-\delta_{\mu,0}-\delta_{\rho,0}}\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2,\sigma_3,\sigma_4=\pm}
	E_{\h q\sigma_4}(X)E^*_{\h q\sigma_3}(0)E_{\h p\sigma_2}(0)E^*_{\h p\sigma_1}(X)\times\\
&\times\tr\left[\gamma_\mu\Delta(\sigma_4)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_3) \gamma_\rho \Delta(\sigma_2) \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2}\Delta(\sigma_1) \right],
\end{split}
\end{equation*}
%
and setting $\mu=0,\,\rho=3$ we have
%
\begin{equation*}
\begin{split}
\mean{\,\h j_{0}(X)\,\h j_3(0)}\ped{B,c}
=& \ii\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2}E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)\times\\
&\times\tr\left[\gamma_0\Delta(\sigma_1)\mathbb{P}_{\chi}\frac{-\I\slashed{\underline{Q}}_{\chi}^+}{{\underline{Q}^+_{\chi}}^2}
	\Delta(\sigma_2) \gamma_3 \frac{-\I\slashed{\underline{P}}_\chi^+}{{\underline{P}^+_\chi}^2} \right].
\end{split}
\end{equation*}
%
The trace is the same of the one computed in previous section
%
\begin{equation*}
F_{03}=-\frac{\I}{2}\chi\left[\sigma_1\left(p_0^2-p_3^2+\underline{P}_2\underline{Q}_2\right)+\sigma_2\left(p_0^2-p_3^2-\underline{P}_2\underline{Q}_2 \right) \right].
\end{equation*}
%
The trace does not depend on coordinates and the correlator is
%
\begin{equation*}
\begin{split}
C\apic{B}_{0|3|}=&\frac{qB\ii}{2}\sumint_{\h P,\h Q}\sum_{\chi}\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}\int_X \frac{x_2^2}{\beta}
\frac{E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0)}{{\underline{Q}^+_{\chi}}^2{\underline{P}^+_\chi}^2}
F_{03}(p_0,p_3,l_p,l_q,\sigma_1,\sigma_2)
\end{split}
\end{equation*}
%
where for $l_p=0$ we have the constraint $\sigma_1=\sigma_2=\bar{\sigma}$, the same must be imposed for $l_q=0$.
This time the integration on $x_2$ would give a $-\delta''(p_2-q_2)$. We define the auxiliary function
%
\begin{equation*}
\begin{split}
(2\pi)^2\delta_{p_0,q_0}\delta(p_3-q_3)\mathcal{I}\apic{B}_{03}\equiv
\int \frac{\D p_2}{2\pi}\int \frac{\D q_2}{2\pi}\int_X E_{\h q\sigma_1}(X)E^*_{\h p\sigma_1}(X) E^*_{\h q\sigma_2}(0)E_{\h p\sigma_2}(0) \frac{x_2^2}{\beta},
\end{split}
\end{equation*}
%
which reads
%
\begin{equation*}
\mathcal{I}\apic{B}_{03}=\delta_{l_p,l_q}\left(\frac{n_p+1}{2}+\frac{\tilde{n}_p+1}{2}\right)-\delta_{l_p,l_q-1}\sqrt{(n_p+1)(\tilde{n}_p+1)}
	-\delta_{l_p,l_q+1}\sqrt{n_p \tilde{n}_p}
\end{equation*}
%
where again we denoted
%
\begin{equation*}
n_p=l_p+\sigma_1\bar\sigma/2-1/2,\quad \tilde{n}_p=l_p+\sigma_2\bar\sigma/2-1/2.
\end{equation*}
%
Therefore,
%
\begin{equation*}
\begin{split}
C\apic{B}_{0|3}=& \frac{\ii qB}{2} T\sum_{\chi}\int\frac{\D p_3}{(2\pi)^2}T\sum_{\{p_n\}}\sum_{l_p,l_q=0}^\infty\sideset{}{'}\sum_{\sigma_1,\sigma_2=\pm}
	\frac{\mathcal{I}\apic{B}_{03}\,F_{03}}{{\Gamma(l_p)}{\Gamma(l_q)}}.
\end{split}
\end{equation*}
%
Consider the sums on $l_p$ and $l_q$; for $l_p=0$ we have
%
\begin{equation*}
\begin{split}
C_{0|3}^{B,l_p=0}=&-\frac{|qB|}{2}T\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{{\Gamma(0)}}\left[\frac{1}{{\Gamma(1)}}-\frac{1}{{\Gamma(0)}} \right]\\
=&|qB|T\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}	\frac{-p_0^2+p_3^2}{\Gamma(0)\Gamma(1)},
\end{split}
\end{equation*}
%
in the same way for $l_q=0$ and $l_p>0$ we find
%
\begin{equation*}
\begin{split}
C_{0|3}^{B,l_p>0,l_q=0}=&|qB|T\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}	\frac{-p_0^2+ p_3^2}{\Gamma(0)\Gamma(1)}.
\end{split}
\end{equation*}
%
Instead for $l_p>0$ and $l_q>0$ after the sums on $\sigma_1$ and $\sigma_2$:
%
\begin{equation*}
\begin{split}
C_{0|3}^{B,l_p>0,l_q>0}=& \frac{|qB|}{2}T\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_{-\infty}^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\frac{p_0^2-p_3^2}{\Gamma(l_p)}\bigg[\frac{1}{{\Gamma(l_p)}}-\frac{1}{{\Gamma(l_p+1)}}-\frac{1-\delta_{l_p,1}}{{\Gamma(l_p-1)}}\bigg]\\
=& |qB|T\sum_{l_p=1}^\infty\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}
	\bigg[\frac{-2p_0^2 +2 p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}+\frac{p_0^2 - p_3^2}{\Gamma(l_p)^2}\bigg];
\end{split}
\end{equation*}
%
all together
%
\begin{equation*}
\begin{split}
C_{0|3}\apic{B}=& |qB|T\sum_{\chi}\chi\int_0^\infty\frac{\D p_3}{(2\pi)^2} T\sum_{\{p_n\}}\Bigg\{\frac{-2 p_0^2+ 2 p_3^2}{\Gamma(0)\Gamma(1)}
	+\sum_{l_p=1}^\infty \bigg[\frac{-2p_0^2 +2 p_3^2}{\Gamma(l_p)\Gamma(l_p+1)}+\frac{p_0^2 - p_3^2}{\Gamma(l_p)^2}\bigg]\Bigg\}.
\end{split}
\end{equation*}
%



==> Interacting.tex <==
\chapter{Interacting fermions}
\label{ch:Interacting}
\section{General properties}
(PASTED FROM NOTES)
We now consider a situation where a dynamical gauge field is present and we ask if any corrections to CME and CSE is possible.
The lagrangian of the theory is
%
\begin{equation*}
\mathcal{L}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}+\bar{\psi}\gamma^\mu\I\left[\de_\mu+q\left(A_\mu\apic{Ext}+A_\mu\right) \right]\psi.
\end{equation*}
%
The partition function of Matsubara finite temperature and density field theory is (in covariant gauge)
%
\begin{equation*}
\mathcal{Z}=C\int \mathcal{D}A_\mu \mathcal{D}\bar{c}\mathcal{D}c \mathcal{D}\bar{\psi}\mathcal{D}\psi  \E^{-S\ped{E}}
\end{equation*}
%
with
%
\begin{equation*}
\begin{split}
S\ped{E}=\int_X \Bigg\{&\frac{1}{4}F^{\mu\nu}F_{\mu\nu} +\frac{1}{2\xi}\de_\mu A_\mu \de_\nu A_\nu+(\de_\mu\bar{c})(\de_\mu+eA_\mu)c+\\
&+\bar{\psi}\gamma_\mu\left[\de_\mu+q\left(A_\mu\apic{Ext}+A_\mu\right) \right]\psi-\mu\ped{A}\bar{\psi}\gamma_0\gamma_5\psi\Bigg\}.
\end{split}
\end{equation*}
%
According to this method the mean value of the current is given by:
%
\begin{equation*}
\mean{\h{j}_\mu(X)}
=\lim_{X_1,X_2\to X} (-\ii)^{1-n_\mu}\left(\gamma_\mu\right)_{ab}\mean{\h{\bar{\psi}}_a(X_1)\h{\psi}_b(X_2)}.
\end{equation*}
%
Therefore any corrections to the Dirac propagator can lead to modifications to the CME conductivity.
According to \cite{Leung:2005yq} at zero temperature and density the exact Dirac propagator has the form:
%
\begin{equation*}
S\ped{F}(x,x')=\sumint_{\h P} E_{\h p}(x) \frac{1}{\gamma\cdot \underline{p}+\Sigma(\underline{p})} \bar{E}_{\h p}(x')
\end{equation*}
%
where the mass operator have the form:
%
\begin{equation*}
\Sigma(\underline{P})=\Sigma_\parallel(\underline{p})\underline{p}_\parallel\cdot\gamma_\parallel
+\Sigma_\perp(\underline{p})\underline{p}_\perp\cdot\gamma_\perp +B(\underline{p})
\end{equation*}
%
and the functions $\Sigma_\parallel,\Sigma_\perp$ and $B$ depend only on $\underline{p}_\parallel^2=-p_0^2+p_3^2$ and on $\underline{p}_\perp^2=2|qB|l$.
So the Euclidena exact propagator at finite temperature and density can be written as
%
\begin{equation*}
\mean{\bar{\Psi}(X)_a \Psi(Y)_b}=-\sumint_{\h P}\sum_\chi E_{\h p}(Y)_{bb'}
\left(\mathbb{P}_\chi\,S\ped{F}(\underline{P}^+_\chi) \right)_{b'a'} \bar{E}_{\h p}(X)_{a'a}.
\end{equation*}
%
with
%
\begin{equation*}
S\ped{F}(\underline{P})=\frac{-\I [1+\Sigma_\parallel(\underline{P})]\slashed{\underline{P}}_\parallel-\I [1+\Sigma_\perp(\underline{P})]\slashed{\underline{P}}_\perp+B(\underline{P})}{[1+\Sigma_\parallel(\underline{P})]^2\underline{P}_\parallel^2+[1+\Sigma_\perp(\underline{P})]^2\underline{P}_\perp^2+B(\underline{P})^2}.
\end{equation*}
%
Repeating the steps in Section \ref{sec:CME} we obtain that the electric current along the magnetic field gets contribution only from the LLL and it is given by:
%
\begin{equation*}
\mean{\h{j}_3(X)}\ped{LLL}= \int_{-\infty}^\infty\frac{\bar\sigma|qB|\D p_3}{(2\pi)^2}\sum_\chi T\sum_{\{\omega_n\}}
\frac{\chi\I [1+\Sigma_\parallel(\underline{P})](\omega_n+\I\mu_\chi)}{[1+\Sigma_\parallel(\underline{P})]^2(\omega_n+\I\mu_\chi)^2+[1+\Sigma_\perp(\underline{p})]^2p_3^2+B(\underline{P})^2},
\end{equation*}
%
which of course can give modification to CME conductivity.

\subsection{Self-energy correction}
Let's evaluate the correction at first order. We have to compute how the propagator is modified.
We have
%
\begin{equation*}
\mean{\bar{\Psi}(X)_a \Psi(Y)_b}=\frac{\int\left(\mathcal{D}\cdots\right) \bar{\Psi}(X)_a \Psi(Y)_b\E^{-S\ped{E}}}{\int\left(\mathcal{D}\cdots\right) \E^{-S\ped{E} } }
\end{equation*}
%
and we separate between a free action and the interaction action:
%
\begin{equation*}
S\ped{E}=S_0+S\ped{I},\quad
S\ped{I}=q\int_Z \bar{\psi}(Z)\gamma_\mu A_\mu(Z) \psi(Z).
\end{equation*}
%
Perturbing on $S\ped{I}$ we obtain
%
\begin{equation*}
\begin{split}
\mean{\bar{\Psi}(X)_a \Psi(Y)_b}
=&\frac{\int\left(\mathcal{D}\cdots\right) \bar{\Psi}(X)_a \Psi(Y)_b\E^{-S_0-S\ped{I}}}{\int\left(\mathcal{D}\cdots\right) \E^{-S_0-S\ped{I}}}\\
=&\frac{\int\left(\mathcal{D}\cdots\right) \bar{\Psi}(X)_a\Psi(Y)_b\E^{-S_0}(1-S\ped{I}+\frac{1}{2}S\ped{I}+\cdots)}
	{\int\left(\mathcal{D}\cdots\right)\E^{-S_0}(1-S\ped{I}+\frac{1}{2}S\ped{I}+\cdots)}\\
=&\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0-\left(\mean{\bar{\Psi}(X)_a \Psi(Y)_b S\ped{I}}_0-\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0\mean{S\ped{I}}_0 \right)\\
&+\frac{1}{2}\left(2\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0 \mean{S\ped{I}}_0\mean{S\ped{I}}_0 -\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0 \mean{S\ped{I}^2}_0\right.\\
&\left. -2\mean{\bar{\Psi}(X)_a \Psi(Y)_b S\ped{I}}_0 \mean{S\ped{I}}_0+\mean{\bar{\Psi}(X)_a \Psi(Y)_b S\ped{I}^2}_0\right)+\cdots
\end{split}
\end{equation*}
%
Since $\mean{S\ped{I}}_0=0$ and $\mean{\bar{\Psi}(X)_a \Psi(Y)_b S\ped{I}}_0=0$ we simply have
%
\begin{equation*}
\mean{\bar{\Psi}(X)_a \Psi(Y)_b}=\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0
+\frac{1}{2}\left( \mean{\bar{\Psi}(X)_a \Psi(Y)_b S\ped{I}^2}_0-\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0 \mean{S\ped{I}^2}_0\right)
\end{equation*}
%
Let us call the second term $G(X,Y)$.
%%
%\begin{equation*}
%\mean{\bar{\Psi}(X)_a \Psi(Y)_b}=\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0
%	+\int\di^4 X'\int\di^4 Y' \mean{\bar{\Psi}(X)_a \Psi(X')_{a'}}_0\Sigma(X',Y')_{a'b'}\mean{\bar{\Psi}(Y')_{b'} \Psi(Y)_b}_0
%\end{equation*}
%%
%where the free propagator is given by Eq.~(\ref{eq:PropinB}) and the self energy is evaluated as~\cite{Ritus:1972ky}
%%
%\begin{equation*}
%\begin{split}
%\Sigma(X,Y)_{ab}=&-\Sigma(Y,X)_{ba}=-\Sigma^{(1)}(Y,X)_{ba}-\Sigma^{(2)}(Y,X)_{ba}\\
%&=-q^2 (\gamma_\rho)_{bb'}\mean{\Psi(Y)_{b'} \bar{\Psi}(X)_{a'} }_0(\gamma_\lambda)_{a'a}\mean{A_\rho(Y) A_\lambda(X)}_0
%	-q^2(\gamma_\rho)_{ba} \mean{A_\rho(Y) A_\lambda(X)}_0 \tr\left[\gamma_\lambda \mean{\Psi(Y) \bar{\Psi}(X) }_0 \right]
%\end{split}
%\end{equation*}
%%
We begin evaluating $G(X,Y)$.
%
\begin{equation*}
\begin{split}
G(X,Y)=&\frac{q^2}{2}\int_{X'}\int_{Y'} (\gamma_\rho)_{cd}(\gamma_\lambda)_{ef}\Big(
\mean{\bar{\Psi}(X)_a \Psi(Y)_b \bar{\Psi}(X')_c A_\rho(X') \Psi(X')_d \bar{\Psi}(Y')_e A_\lambda(Y') \Psi(Y')_f }_0\\
&-\mean{\bar{\Psi}(X)_a \Psi(Y)_b}_0\mean{ \bar{\Psi}(X')_c A_\rho(X') \Psi(X')_d \bar{\Psi}(Y')_e A_\lambda(Y') \Psi(Y')_f }_0\Big).
\end{split}
\end{equation*}
%
Using Wick's theorem we obtain
%
\begin{equation*}
\begin{split}
G(X,Y)_{ab}=\frac{q^2}{2}\int_{X'}\int_{Y'} (\gamma_\rho)_{cd}(\gamma_\lambda)_{ef}\mean{A_\rho(X')A_\lambda(Y')}_0\big(&
\mean{\bar{a}f}\mean{\bar{e}d}\mean{\bar{c}b}-\mean{\bar{a}d}\mean{\bar{e}f}\mean{\bar{c}b}+\\
&-\mean{\bar{a}f}\mean{\bar{c}d}\mean{\bar{e}b}+\mean{\bar{a}d}\mean{\bar{c}f}\mean{\bar{e}b}\big)
\end{split}
\end{equation*}
%
The electric current correction is
%
\begin{equation*}
\begin{split}
\mean{\h{j}_3(X)}=&\mean{\h{j}_3(0)}=-\ii\lim_{X_1,X_2\to 0} \left(\gamma_3\right)_{ab}G(X_1,X_2)_{ab}
	=\frac{\ii q^2}{2}\lim_{X_1,X_2\to 0} \int_{X'}\int_{Y'} \mean{A_\rho(X')A_\lambda(Y')}_0\times\\\
&\times\left\{\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(Y')}\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(X_1)}\right]\right.\\
&-\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(X_1)}\right]
\tr\left[\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(Y')}\right]\\
&-\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(Y')}\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(X_1)}\right]
\tr\left[\gamma_\rho\mean{\Psi(X')\bar{\Psi}(X')}\right]\\
&\left.+\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(Y')}\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(X_1)}\right] \right\}.
\end{split}
\end{equation*}
%
Using the symmetric properties of photon propagator: $ \mean{A_\rho(X')A_\lambda(Y')}_0= \mean{A_\lambda(X')A_\rho(Y')}_0= \mean{A_\rho(Y')A_\lambda(X')}_0$
we have
%
\begin{equation*}
\begin{split}
\mean{\h{j}_3(X)}=&\ii q^2\lim_{X_1,X_2\to 0} \int_{X'}\int_{Y'} \mean{A_\rho(X')A_\lambda(Y')}_0\times\\
&\times\Big\{\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(Y')}\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(X_1)}\right]\\
&-\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(X_1)}\right]
\tr\left[\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(Y')}\right]\Big\}.
\end{split}
\end{equation*}
%
Consider just the first term, it becomes
%
\begin{equation*}
\begin{split}
\mean{\h{j}_3(X)}^{(1)}&=\ii q^2\lim_{X_1,X_2\to 0} \int_{X'}\int_{Y'} \mean{A_\rho(X')A_\lambda(Y')}_0\times\\
&\times\tr\left[\gamma_3 \mean{\Psi(X_2)\bar{\Psi}(X')}\gamma_\rho\mean{\Psi(X')\bar{\Psi}(Y')}\gamma_\lambda\mean{\Psi(Y')\bar{\Psi}(X_1)}\right]	.
\end{split}
\end{equation*}
%
The photon propagator is
%
\begin{equation*}
\mean{A_\rho(Y) A_\lambda(X)}_0=\sumint_{K}\E^{\I(Y-X)\cdot K}\frac{1}{K^2}\left(\delta_{\rho\lambda}+(1-\xi)\frac{K_\rho K_\lambda}{K^2}\right).
\end{equation*}
%
\section{Universality of CME}
CME no mass or UV correction~\cite{Fukushima:2012vr}
\section{Non-Universality of AVE}
Radiative correction to chiral separation effect~\cite{Gorbar:2013upa}.
%******************************************************************
\section{Two-loop QED correction to AVE conductivity}
%******************************************************************
Consider a QED plasma of massless fermions with the Lagrangian density
%
\begin{equation*}
\mathcal{L}=-\frac{1}{4}F^{\mu\nu}F_{\mu\nu}-\I\bar{\psi}\gamma^\mu D_\mu\psi
\end{equation*}
%
where $F_{\mu\nu}=\de_\mu A_\nu-\de_\nu A_\mu$ is the electromagnetic field strength tensor associated with the gauge field $A_\mu$ and $D_\mu=\de_\mu-\I e A_\mu$ is the covariant derivative.
The corresponding symmetric stress-energy tensor is
%
\begin{equation*}
\begin{split}
\h T_{\mu\nu}=&F_\mu^{\,\rho}F_{\nu\rho}-\frac{1}{4}\eta_{\mu\nu}F^{\rho\lambda}F_{\rho\lambda}\\
&+\frac{1}{2}\left(\bar{\psi}\gamma_{(\mu}D_{\nu)}\psi-D_{(\mu}\bar{\psi}\gamma_{\nu)}\psi\right).
\end{split}
\end{equation*}
%
The axial current $\h j_5^\mu=\bar{\psi}\gamma^\mu\gamma^5\psi$ because of the gauge interactions is not conserved but is anomalous:
%
\begin{equation}
\label{axialanom}
\de_\mu \h j_5^\mu=-\frac{e^2}{16\pi^2}\epsilon^{\mu\nu\rho\sigma}F_{\mu\nu}F_{\rho\sigma}.
\end{equation}
%

In the density matrix formalism, when the system is at global thermal equilibrium with a inverse four-temperature $\beta^\mu=u^\mu/T$ possessing a non-vanishing thermal vorticity
and a chemical potential $\mu$ related to the conserved electric charge of fermions,
the CVE conductivity $\sigma_5\apic{V}$ is computed using the following formula in the imaginary time formalism \cite{Buzzegoli:2017cqy}:
%
\begin{equation}
\label{coeffCVE}
\begin{split}
\sigma_5\apic{V} %=&\int_0^{|\beta|}\D \tau \,\mean{\,\h J^{\,3}_{-\I \tau}\,\h j^{\,3}_5(0)\,}_{T,c} \\
=&\int_0^{|\beta|}\D \tau\int \D^3 x \left(\mean{\h T^{02}(\tau ,\vec x) \h j^{\,3}_{5}(0)}_{T,c} x^1\right.\\
&\left. - \mean{\h T^{01}(\tau ,\vec x)\h j^{\,3}_{5}(0)}_{T,c}x^2\right)\\
\equiv & C^{02|3|1}-C^{01|3|2}
\end{split}
\end{equation}
%
where the subscript $c$ in the correlators stands for connected quantities and we denote the mean values in rest frame with a subscript $T$, that is:
%
\begin{equation*}
\mean{\cdots}_{T}=\frac{\tr\left[\exp\left(-\frac{\h H}{T}+\frac{\mu}{T}\h Q\right)\cdots\right]}{\tr\left[\exp\left(-\frac{\h H}{T}+\frac{\mu}{T}\h Q\right)\right]}.
\end{equation*}
%

The main ingredient in eq.~(\ref{coeffCVE}), as in the corresponding Kubo formula~\cite{Amado:2011zx}, is the correlator between th axial current density and energy flux density.
Following a Coleman-Hill like argument it has been shown in \cite{Golkar:2012kb,Hou:2012xg} that the only two-loop contribution to that correlator comes only from those that include the anomalous triangular subdiagram
, Fig.~\ref{fig:FeynDiag2loop}. This means that only the gauge part of the stress-energy tensor gives corrections to the CVE conductivity.
%
\begin{figure}[thb!]
	\centering
	\subfigure[Anomalous diagram]{\label{fig:FeynDiag2loop}\includegraphics[width=0.45\columnwidth]{FeynDiag2loop.png}}
	\subfigure[Effective diagram]{\label{fig:FeynDiagEff}\includegraphics[width=0.45\columnwidth]{FeynDiagEff.png}}
	\caption{(a) The leading order diagram and (b) the same diagram after replacing the effective vertex, representing the anomalous effect of the triangle diagram.}
	\label{fig:FeynDiag}
\end{figure}
%

Moreover, since the triangle part is constrained by the anomalous Ward identity~(\ref{axialanom}) we can effectively reduce to one-loop calculation by replacing the triangle part of the diagram with the effective
vertex~\cite{Golkar:2012kb}, Fig.~\ref{fig:FeynDiagEff}:
%
\begin{equation*}
\h j^\mu\ped{Anom}=-\frac{e^2}{4\pi^2}\epsilon^{\mu\nu\lambda\sigma}A_\nu\de_\lambda A_\sigma.
\end{equation*}
%

To calculate the latter two terms in~(\ref{coeffCVE}) we write the correlation functions in the Euclidean form.
Before doing that we introduce the notation:
%
\begin{equation*}%\label{symbols}
P=(p_n, {\vec p} ),\quad X=(\tau ,{\vec x}), 
\quad \sumint_{P}=\frac{1}{|\beta|}\sum_{p_n=-\infty}^\infty\int \frac{\D ^3 p }{(2\pi)^3}
\end{equation*}
%
and: 
%
\begin{equation*}
\tilde\delta(P)=\int_0^{|\beta|}\D \tau\int \D^3 x \,\E^{\I X\cdot P}=|\beta| (2\pi)^3 \delta_{p_n,0}\,\delta^{(3)}({\vec p})
\end{equation*}
%
where $X\cdot P=\tau\,p_n-{\vec x}{\vec p}$ and $p_n=2\pi n /|\beta|$ are the Matsubara frequencies.
The photon propagator in the imaginary time reads \cite{KapustaGale,Laine:2016hma}:
%
\begin{equation}\label{photprop}
\mean{ {\rm T}_\tau A_\mu(X)A_\nu(Y)}_T= \sumint_{P}\E^{\I P(X-Y)} \frac{G_{\mu\nu}(P)}{P^2}
\end{equation}
%
where:
%
\begin{equation*}%\label{propden}
G_{\mu\nu}(P) = \delta_{\mu,\nu}+(1-\zeta)\frac{P_\mu P_\nu}{P^2}
\end{equation*}
%
and $P^2$ is the Euclidean squared magnitude of the four vector $P$.

The Euclidean effective axial current using the point splitting procedure reads:
%
\begin{equation*}
\begin{split}
\h j&\ped{Anom}^\alpha(X)=-\frac{e^2}{4\pi^2}\epsilon^{\alpha\nu\lambda\sigma}A_\nu(X)\de_\lambda A_\sigma(X)\\
&=\lim_{X_1,X_2\to X} \frac{e^2}{8\pi^2}\epsilon^{\alpha\rho\lambda\tau}(\de_{X_1\lambda}-\de_{X_2\lambda}) A_\rho(X_1)A_\tau(X_2)\\
&\equiv\mathcal{J}\ped{Anom}^{\alpha,\,\rho\tau}(\de_{X_1},\de_{X_2})A_\rho(X_1)A_\tau(X_2).
\end{split}
\end{equation*}
%
Instead the electromagnetic stress-energy tensor is
%
\begin{equation*}
\h T\ped{em}^{\mu\nu}(X)=\lim_{X_1,X_2\to X} \mathcal{D}\ped{em}^{\mu\nu,\,\rho\sigma}(\de_{X_1},\de_{X_2})A_\kappa(X_1)A_\sigma(X_2)
\end{equation*}
%
with 
%
\begin{equation*}
\begin{split}
\mathcal{D}\ped{em}^{\mu\nu,\,\kappa\sigma}(\de_{X_1},\de_{X_2})=&\frac{1}{2}\left[\delta^{\kappa,\sigma}\!\left(\de^\mu_{X_1}\de^\nu_{X_2}\!+\!\de^\nu_{X_1}\de^\mu_{X_2}\right) \right.\\
&-\!\left(\delta^{\sigma,\nu}\de^\mu_{X_1}\de^\kappa_{X_2}+\delta^{\kappa,\nu}\de^\sigma_{X_1}\de^\mu_{X_2}\right)\\
&\!-\!\left(\delta^{\kappa,\mu}\de^\sigma_{X_1}\de^\nu_{X_2} \!+\!\delta^{\sigma,\mu}\de^\nu_{X_1}\de^\kappa_{X_2}\right)\\
&+\left(\delta^{\kappa,\mu}\delta^{\sigma,\nu}\!+\!\delta^{\kappa,\nu}\delta^{\sigma,\mu}\right)\de_{X_1}\!\!\!\cdot\!\de_{X_2}\\
&\left.\!\!-\!\eta^{\mu\nu}\!\left(\delta^{\kappa,\sigma}\de_{X_1}\!\!\!\cdot\!\de_{X_2}\!-\!\de^\sigma_{X_1}\de^\kappa_{X_2}\right)\right].
\end{split}
\end{equation*}
%

Now we are ready to evaluate the two-loop correction of the coefficient
%
\begin{equation}\label{Archetype}
C^{\mu\nu\alpha i}=\int_0^{|\beta|}\D \tau\int \D^3 x \mean{\h T^{\mu\nu}(X) \h j^{\,\alpha}_{5}(0)}_{T,c} x^i.
\end{equation}
%
First, we consider:
%
\begin{equation*}
\begin{split}
&\mean{{\rm T}_\tau \h T^{\mu\nu}(X)\h j\ped{Anom}^\alpha(Y)}_{T,c}=\lim_{\substack{X_1,X_2\to X \\ Y_1,Y_2\to Y}}
\mathcal{D}\ped{em}^{\mu\nu,\,\kappa\sigma}(\partial_{X_1},\partial_{X_2})\\
&\cdot \mathcal{J}\ped{Anom}^{\alpha,\,\rho\tau}(\partial_{Y_1},\partial_{Y_2}) \mean{{\rm T}_\tau A_\kappa(X_1)A_\sigma(X_2)A_\rho(Y_1)A_\tau(Y_2)}_{T,c}.
\end{split}
\end{equation*}
%
The evaluation of the four gauge field correlator can be done by employing the standard Wick 
theorem and since only its connected part appears, only the following two terms survive:
%
\begin{equation*}
\begin{split}
\mean{A_1 A_2 A_3 A_4}_{c}&=\mean{A_1 A_2 A_3 A_4}-\mean{A_1 A_2}\mean{A_3 A_4}\\
&=\mean{A_1 A_3}\mean{A_2 A_4} + \mean{A_1 A_4}\mean{A_2 A_3}.
\end{split}
\end{equation*}
%
It can be shown that these two latters terms give the same contribution, therefore we consider just the first one.
The only correlators left are the already known two point correlators of the photon; in the Fourier space we can choose the 
following notation to express them as in~(\ref{photprop})
%
\begin{gather*}
\mean{ {\rm T}_\tau A_\kappa(X_1)A_\rho(Y_1)}_T= \sumint_{P}\E^{\I P(X_1-Y_1)} \frac{G_{\kappa\rho}(P)}{P^2},\\
\mean{ {\rm T}_\tau A_\sigma(X_2)A_\tau(Y_2)}_T= \sumint_{Q}\E^{\I Q(X_2-Y_2)} \frac{G_{\sigma\tau}(Q)}{Q^2}.
\end{gather*}
%
Since the coordinate dependence is now only in the exponential factor, the derivative action present in the operators $\mathcal{D}\ped{em}$ and $\mathcal{J}\ped{Anom}$
is easily found:
%
\begin{gather*}
\de_X \mean{ {\rm T}_\tau A_\mu(X)A_\nu(Y)}_T= \I P\mean{ {\rm T}_\tau A_\mu(X)A_\nu(Y)}_T;\\
\de_Y \mean{ {\rm T}_\tau A_\mu(X)A_\nu(Y)}_T= - \I P\mean{ {\rm T}_\tau A_\mu(X)A_\nu(Y)}_T.
\end{gather*}
%
With these substitutions and after the limit of $X_1,X_2\to X$ and $Y_1,Y_2\to Y$ the correlator in $Y=0$ becomes
%
\begin{equation*}
\begin{split}
\mean{{\rm T}_\tau &\h T^{\mu\nu}(X)\h j\ped{Anom}^\alpha(0)}_{T,c}=\sumint_{P,Q}\frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}\E^{\I (P+Q)\cdot X},
\end{split}
\end{equation*}
%
where the function $F^{\mu\nu\alpha}$ results from of the composite operator in the correlation functions, 
in this case:
%
\begin{equation}\label{Ffunz}
\begin{split}
&F^{\mu\nu\alpha}(P, Q)=\\&2 \mathcal{D}\ped{em}^{\mu\nu,\,\kappa\sigma}(\I P,\I Q )\mathcal{J}\ped{Anom}^{\alpha,\,\rho\tau}(-\I Q,-\I P ) G_{\kappa\rho}(P)G_{\sigma\tau}(Q)\\
&=\frac{\I e^2}{8\pi^2}\left[\left(P_\mu-Q_\mu\right)\epsilon_{\alpha\nu\rho\sigma}P_\rho Q_\sigma+\left(P_\nu-Q_\nu\right)\epsilon_{\alpha\mu\rho\sigma}P_\rho Q_\sigma\right].
\end{split}
\end{equation}
%

So the coefficient (\ref{Archetype}) becomes
%
\begin{equation*}
C^{\mu\nu\alpha i}=\int_0^{|\beta|}\D \tau\int \D^3 x \sumint_{P,Q}\E^{\I(P+Q)X}x^i \frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}
\end{equation*}
%
and rewriting the coordinate $x^i$ as derivative of the exponential and integrating by part
%
\begin{equation*}
\begin{split}
C^{\mu\nu\alpha i} &= -\I\int_0^{|\beta|}\!\!\!\!\D \tau\!\!\!\int \D^3 x \sumint_{P,Q}\left(\frac{\de}{\de q_i}\E^{\I(P+Q)X}\right) \frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}\\
&= \I\!\sumint_{P,Q}\!\int_0^{|\beta|}\!\!\!\!\D \tau\!\!\!\int \D^3 x \,\E^{\I(P+Q)X}\!\! \left(\frac{\de}{\de q_i}\frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}\right).
\end{split}
\end{equation*}
%
At this point the integral over the coordinates gives a $\tilde\delta(P+Q)$, that we can use to sum over the momentum $Q$
%
\begin{equation*}
C^{\mu\nu\alpha i} = \I\sumint_{P}\left(\frac{\de}{\de q_i}\frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}\right)_{Q=-P}.
\end{equation*}
%

The derivative of the quantity in the bracket is simplified by the property $F^{\mu\nu\alpha}(P,-P)=0$, as we see from~(\ref{Ffunz}):
%
\begin{equation*}
\begin{split}
\left(\frac{\de}{\de q_i}\frac{F^{\mu\nu\alpha}(P,Q)}{P^2 Q^2}\right)_{Q=-P}&=\frac{1}{P^4}\left(\frac{\de}{\de q_i}F^{\mu\nu\alpha}(P,Q)\right)_{Q=-P}\\
&\equiv \frac{f^{\mu\nu\alpha i}(p_n,\vec p)}{(p_n^2+{\vec p}^2)^2},
\end{split}
\end{equation*}
%
where we have defined the function $f^{\mu\nu\alpha i}(p_n,\vec p)$, that is a polynomial function. For instance we need
%
\begin{equation*}
f^{0132}=\frac{\I e^2}{4\pi^2}(p_n^2-{p^{1}}^2),f^{0231}=-\frac{\I e^2}{4\pi^2}(p_n^2-{p^{2}}^2).
\end{equation*}
%

We are then reduced to a single momentum integral that can be made explicly with standard technique.
Consider first
%
\begin{equation*}
\begin{split}
C^{0132}&=-\frac{e^2}{4\pi^2}\int\D p \frac{1}{\beta}\sum_{p_n}\int_{4\pi} \frac{\D \Omega_p}{(2\pi)^3}\frac{p^2(p_n^2-p_{1}^2)}{(p_n^2+{\vec p}^2)^2}\\
& =-\frac{e^2}{8\pi^4}\int\D p \frac{1}{\beta}\sum_{p_n}\frac{p^2(p_n^2-p^2/3)}{(p_n^2+{\vec p}^2)^2}\\
& =-\frac{e^2}{24\pi^4}\int\D p \left(p\, n\ped{B}(p)+2p^2 n\ped{B}'(p)\right),
\end{split}
\end{equation*}
%
where $n\ped{B}$ is the Bose-Einstein distribution function
%
\begin{equation*}
n\ped{B}(p)=\frac{1}{\E^{\beta p}-1}
\end{equation*}
%
and $n\ped{B}'(p)$ its derivative that can be integrated by parts:
%
\begin{equation*}
\int\D p 2p^2 n\ped{B}'(p)=-4 \int\D p \,p\, n\ped{B}(p).
\end{equation*}
%
At the end we are left with
%
\begin{equation*}
\begin{split}
C^{0132}&=\frac{e^2}{8\pi^4}\int\D p \,p\, n\ped{B}(p)=\frac{e^2}{48\pi^2}T^2.
\end{split}
\end{equation*}
%
In the same way we can show that $C^{0231}=-C^{0132}$ so that the two-loop correction of~(\ref{coeffCVE}) is
%
\begin{equation}
\sigma_5\apic{V(2)}=\frac{e^2}{24\pi^2}T^2.
\end{equation}
%
Our result is twice the value of \cite{Hou:2012xg,Golkar:2012kb} because we have considered both right and left fermions contribution instead that just one chirality.
\section{Equivalence principle at finite temperature}
